PromptWizard: Task-Aware Prompt Optimization Framework

Large language models (LLMs) have transformed AI across diverse domains, with prompting being central to their success in guiding model outputs. However, manual prompt engineering is both labor-intensive and domain-specific, necessitating the need for automated solutions. We introduce PromptWizard, a novel, fully automated framework for discrete prompt optimization, utilizing a self-evolving, self-adapting mechanism. Through a feedback-driven critique and synthesis process, PromptWizard achieves an effective balance between exploration and exploitation, iteratively refining both prompt instructions and in-context examples to generate human-readable, task-specific prompts. This guided approach systematically improves prompt quality, resulting in superior performance across 45 tasks. PromptWizard excels even with limited training data, smaller LLMs, and various LLM architectures. Additionally, our cost analysis reveals a substantial reduction in API calls, token usage, and overall cost, demonstrating PromptWizard's efficiency, scalability, and advantages over existing prompt optimization strategies.

==> 5-results.tex <==
\vspace{-15pt}
\section{Results}
\label{sec:results}
% We extensively evaluate \prompt's performance on \red{35 tasks} from popular benchmarks across domains, comparing it against SOTA foundational models and prompt optimization approaches.
\subsection{Performance Analysis Against Various Prompting Baselines}
\label{sec:perf}
\vspace{-5pt}
Table~\ref{tab:perf} presents the performance comparison of \prompt against state-of-the-art foundational models like \gpt, Gemini ultra and prompt optimization approaches such as PromptBreeder~\cite{fernando2023promptbreeder} and MedPrompt~\cite{nori2023generalist}. For tasks where baseline models haven't been evaluated, we denote the entries with `--' (not applicable). Across all tasks and datasets, the prompts derived using \prompt consistently outperforms \gpt, Gemini Ultra and PromptBreeder. It's noteworthy that the evaluation is conducted using the same test data and few-shot settings. On average, \prompt achieves nearly \textbf{+$5$\% improvement} over \gpt, Gemini and PromptBreeder, highlighting the effectiveness of our principled approach in prompt synthesis and refinement. Particularly on reasoning tasks like GSM8k, \prompt exhibits a significant performance boost (+$11.9$\%) compared to PromptBreeder, attributed to its ability to synthesize diverse few-shot examples with reasoning steps.

\begin{table}[!t]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{cllllll}
\hline
\multicolumn{1}{l}{}  &                                     & PB*   & GPT 4* & Gemini*    & Medprompt*     & PW (ours)     \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{General domain}} & \multicolumn{1}{l|}{GSM8k} & 83.5 & 92.0 & 94.4 & --            & \textbf{95.4} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{CSQA}           & 85.9 & --    & --         & --            & \textbf{86.4} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{SQA}            & 80.2 & --    & --         & --            & \textbf{80.8} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{Ethos}          & 89.0 & --    & --         & --            & \textbf{89.4} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{BBH (23)}            & --   & --    & 83.6       & --            & \textbf{88.1} \\ \hline
% \multicolumn{1}{c|}{} & \multicolumn{1}{l|}{MMLU} & --   & 86.4  & 90.04 (32) & 90.1 (32)     &       \red{XXX}        \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Medical}}        & \multicolumn{1}{l|}{MedQA} & --   & 81.4 & --   & \textbf{90.2} & 84.4          \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{PubMedQA}       & --   & 75.2  & --         & \textbf{82.0} & 78.2          \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{MMLU - Med (6)}     & --   & 87.4  & --         & \textbf{94.3} & 89.5          \\ \hline
\end{tabular}
}
\caption{PromptWizard (PW) comparison to state-of-the-art foundational models (GPT 4~\cite{openai2024gpt4} and Gemini Ultra~\cite{geminiteam2024gemini}) and prompt optimization approaches (PB: PromptBreeder~\cite{fernando2023promptbreeder} and MedPrompt~\cite{nori2023generalist}).\\ * sourced directly from the original reports.}
\label{tab:perf}
\vspace{-15pt}
\end{table}
We compare the efficacy of \prompt with MedPrompt, that is evaluated mostly on medical domain datasets. While \prompt achieves comparable performance to MedPrompt on datasets like PubMedQA, MedQA, and MMLU-6 medical tasks, it does so at significantly lower computational and latency costs. Specifically, \prompt requires only $139$ LLM calls (see Algo~\ref{algo:cost}) to achieve the current accuracy, whereas MedPrompt makes $73.2$ times more LLM calls in MedQA, $3.5$ times more in PubMedQA, and $1.1$ times more in MMLU medical datasets during preprocessing. Additionally, during the inference step, MedPrompt makes $5$ times more calls than \prompt for each new query. This is because MedPrompt generates offline COT reasoning for all train/dev/val examples during preprocessing with MedQA having 10k+ train examples, PubMedQA with 500, and MMLU has 153 examples. In contrast, we use just 25 examples (5 mini-batch to select diverse examples and then synthesize them further). Moreover, during inference, \prompt does just 1 LLM call as compared to 5 calls per query for MedPrompt.   
It's important to note that our baseline comparison is limited to PromptBreeder and MedPrompt, as the other baseline numbers from APE, APO, EvoPrompt, PromptAgent, and OPRO are significantly lower. Appendix~\ref{app:bestprompts} shows final best prompts with few-shot examples for each dataset.
%See Appendix~\ref{sec:} and~\ref{} for train/test splits and hyper parameters used.  

\textbf{Summary:} \textit{\prompt demonstrates the ability to generate effective prompt instructions and few-shot examples with reasoning across various tasks and datasets, outperforming popular baselines while maintaining significantly reduced computational and latency overheads.}


\begin{table*}[!t]
\begin{minipage}[l]{0.33\linewidth}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lll}
\hline
Datasets      & 5 (eg) & 25 (eg) \\ \hline
MMLU- physics & 75.5   & 79.4    \\
GSM8k         & 94.0   & 95.4    \\
Ethos         & 86.4   & 89.4    \\
PubMedQA      & 68.0   & 78.2    \\
MedQA         & 80.4   & 82.9    \\ \hline
Average       & 80.9   & 85.0    \\ \hline
\end{tabular}%
}
% \caption{}
% \label{tab:my-table}
        \caption{\prompt's performance with 5 examples.}
        \label{tab:fewer}
        \vspace{-5pt}
\end{minipage}
~~
\begin{minipage}[l]{0.3\linewidth}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lll}
\hline
Datasets        & \llama & \gpt \\ \hline
GSM8k   & 94.6      & 95.4 \\
Ethos   & 89.2      & 89.4 \\\hline
% PubMed  &  \red{xxx}         & 78.2 \\
% MedQA   &   \red{xxx}        & 82.9 \\ \hline
Average & {91.9}      & 92.4 \\ \hline
\end{tabular}%
}
% \caption{}
% \label{tab:my-table}
        \caption{Performance with smaller LLMs.}
        \label{tab:small}
        \vspace{-5pt}
\end{minipage}
~~
\begin{minipage}[l]{0.31\linewidth}

\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\hline
Models          & With PW        & Without PW \\ \hline
\gpt      & \textbf{95.4} & 92         \\
\gptt    & \textbf{75.6} & 57.1       \\
\llama & \textbf{90.2}  & 56.8      
\end{tabular}%
}
% \caption{}
% \label{tab:my-table}
        \caption{Performance with different Base LLMs on GSM8k.}
        \label{tab:base}
        \vspace{-5pt}
\end{minipage}
\vspace{-5pt}
 % \caption{.}
 %        \label{fig:hybrid_results}
        \vspace{-10pt}
\end{table*}
\vspace{-5pt}
\subsection{\prompt Efficacy with Fewer Training Examples}
\label{sec:train_res}
% As described in Section~\ref{sec:method}, \prompt utilizes training samples from the dataset to assess the prompt's effectiveness and to select negative examples, which are then used to synthesize new few-shot examples. 
In real-world situations, data availability can be limited, with tasks changing or lacking curated train/test data. We show how \prompt excels in creating effective prompts using just 3-5 examples, showcasing its efficacy in few-shot learning scenarios.

To simulate this setup, we randomly select \textit{just 5} examples as our training data, which \prompt utilizes for all its evaluations, critics, and the generation of new synthesized examples that are diverse and representative of the tasks. Table~\ref{tab:fewer} presents the effectiveness of \prompt across 5 tasks when provided with only 5 training examples (5 eg) compared to having access to the complete training set (25 eg). Remarkably, \prompt achieves very similar performance, with only a \textbf{$4$\% reduction} in accuracy on average when limited to just 5 random training examples. This effectiveness is primarily attributed to the effective synthetic example generation coupled with a detailed reasoning chain, enabling the prompt to guide the model to generate accurate answers. It's worth noting that to ensure robust evaluation, we report average numbers after three experimental runs.

\textbf{Summary:} \textit{\prompt demonstrates its effectiveness even with a modest number of training examples, making it suitable for scenarios where comprehensive datasets are unavailable.}
\vspace{-5pt}
\subsection{\prompt with Smaller LLMs}
\label{sec:small_res}
Up until now, we've utilized \gpt as the LLM for all components during preprocessing. Here, we assess the effectiveness of \prompt's methodology when LLM agents employ a smaller model such as \llama. It's important to note that the smaller model, \llama, is only utilized during preprocessing to derive an effective prompt alongside few-shot examples and reasoning. During inference, we continue to use the default \gpt as the base LLM. The rationale behind this approach is to significantly reduce computational overhead by using a smaller model during preprocessing, while still relying on a powerful model during inference to maximize task accuracy. 

Table~\ref{tab:small} displays task accuracy across multiple datasets when a smaller model like \llama is employed for the agents, compared to the default \gpt during preprocessing. Notably, the final prompt generated by \prompt using \llama exhibits very comparable performance (<$1$\% accuracy drop) compared to prompts generated using \gpt. This underscores the effectiveness of \prompt's principled methodology and its adaptability to different LLM models.

\textbf{Summary:} \textit{\prompt achieves identical task performance when optimal prompts are generated using a smaller LLM model, demonstrating its versatility and robustness across model sizes.}
\vspace{-5pt}
\subsection{Ablation Analysis}
\label{sec:abl+res}
We conduct two types of ablation analysis: (i) examining the use of different base LLMs, and (ii) assessing the effectiveness of individual stages of \prompt.

\textbf{Different Base LLMs.} We investigate \prompt's performance across different LLMs by experimenting with three scenarios: using \gpt, \gptt, or \llama as both the base LLM (during inference) and the agent LLMs (during preprocessing). Table~\ref{tab:base} displays the model's performance with and without \prompt (PW) on the GSM8k dataset. Notably, with \prompt, we observe improvements in task accuracy across all models, with increases close to +18\% and +33\% for \gptt and \llama models, respectively. For baselines without \prompt, we employ the same setting of few-shot + COT~\cite{touvron2023llama}. Similar trends are observed for other datasets.

\textbf{Summary:} \textit{\prompt can be applied across different classes of LLMs, and our evaluation demonstrates its significant improvement in task performance across various model families.}

\begin{wraptable}{r}{5cm}
\vspace{-2pt}
\resizebox{0.35\textwidth}{!}{%
\begin{tabular}{lll}
\hline
                         & GSM8k          & Ethos          \\ \hline
All                      & \textbf{95.4} & \textbf{89.4} \\
No Mutation and Scoring  & 95.2          & 87.1           \\
No Critic and Synthesize & 90.9          & 86.9          \\
No intent \& Expert      & 95             & 88.7          \\
No Reasoning             & 45.9           & 87.6  \\ \hline        
\end{tabular}%
}
\caption{Abaltion Study}
\label{tab:aba}
\vspace{-8pt}
\end{wraptable}
\textbf{Effectiveness of different stages of \prompt.} 
We now examine the effects of individual stages of our methodology, evaluating each setting with few-shot examples. Table~\ref{tab:aba} illustrates the impact of different stages on \prompt, assessed on GSM8k and Ethos datasets. The mutation and scoring in the first stage (iterative refinement of prompt instruction) can enhance performance by $1-2$\%. Incorporating critic feedback and refinement in this stage further increases performance by $3-5$\%. Furthermore, integrating task intent and expert persona leads to a performance improvement ranging from $0.5-1$\%. Finally, reasoning on few-shot examples emerges as a significant factor in boosting prompt performance across datasets. This ablation study underscores the significance of individual agents within the \prompt framework, as they work collectively to enhance prompt and model performance.

% \textbf{Summary:} \textit{Each stage of the \prompt framework plays a crucial role in improving both prompt and model performance.} 

% After rigorous evaluation across diverse tasks and datasets, we advocate for the optimal prompt strategy for LLMs lies in a fusion of improved prompt instruction (augmented and refined) and strategic few-shot examples bolstered by reasoning, inclusive of negative or synthesized instances, to maximize task performance.







